Using Spatial Pooler of Hierarchical Temporal Memory to classify noisy videos with predefined complexity

This paper examines the performance of a Spatial Pooler (SP) of a Hierarchical Temporal Memory (HTM) in the task of noisy object recognition. To address this challenge, a dedicated custom-designed system based on the SP, histogram calculation module and SVM classifier was implemented. In addition to implementing their own version of HTM, the authors also designed a profiler which is capable of tracing all of the key parameters of the system. This was necessary, since an analysis and monitoring of the system performance turned out to be extremely difficult using conventional testing and debugging tools. The system was initially trained on artificially prepared videos without noise and then tested with a set of noisy video streams. This approach was intended to mimic a real life scenario where an agent or a system trained to deal with ideal objects faces a task of classifying distorted and noisy ones in its regular working conditions. The authors conducted a series of experiments for various macro parameters of HTM SP, as well as for different levels of video reduction ratios. The experiments allowed them to evaluate the performance of two different system setups (i.e. 'Multiple HTMs' and 'Single HTM') under various noise conditions with 32--frame video files. Results of all the tests were compared to SVM baseline setup. It was determined that the system featuring SP is capable of achieving approximately 12 times the noise reduction for a video signal with with distorted bits accounting for 13\% of the total. Furthermore, the system featuring SP performed better also in the experiments without a noise component and achieved a max F1 score of 0.96. The experiments also revealed that a rise of column and synapse number of SP has a substantial impact on the performance of the system. Consequently, the highest F1 score values were obtained for 256 and 4096 synapses and columns respectively.

==> contents-11-system-architecture.tex <==
\subsection{System Architecture}
\label{subsection:system_architecture}

Implemented system architecture is highly modular, enabling continuous enhancements. Written using Python -- object-oriented, high-level language with a rich variety of scientific and utility libraries, with crucial parts progressively replaced by fragments implemented in OpenCL.

The HTM itself is a 'core' module, beside which are ones necessary for the system to function (responsible for data reading and encoding, as well as results interpretation) and ones created for debugging and statistics gathering purposes. Overall system architecture is depicted in (Fig. \ref{fig:architecture_of_the_implemented_system}). The most relevant modules are described in details below.

\begin{figure}[tbp]
\centering
    \includegraphics[width=0.45\textwidth]{figures/system_architecture}
    \caption{Architecture of the implemented system}
    \label{fig:architecture_of_the_implemented_system}
\end{figure}

\subsubsection{Outer Structure}

The outermost level of system is CLI (Command Line Interface). Depending on the provided command line options it invokes particular setup -- either 'Single HTM' or 'Multiple HTMs' mode. In 'Single HTM' mode data from all categories is fed into single HTM instance. 'Multiple HTMs' refers to creating HTM instances on per-category basis, resulting in an ensemble of one-vs-all detectors. In both modes the same wrappers encapsulating the actual processing units can be used. A wrapper is created for particular HTM use -- it is responsible for creating relevant data readers, encoders, decoders and output writers and passing them to the iterator -- a part of core that manages HTM cycles. After data is processed by the wrapper, the result reaches CLI, which is responsible for further analysis and data presentation -- combining wrappers outputs, gathering statistics, training classifier used to provide final results, rendering data visualizations etc.

Current experiment is conducted using 'Multiple HTMs' mode. Each wrapper creates reader able to get data from video files and encoder that converts raw frame data to the required format. HTM output is neither modified (pass-through decoder module) nor stored for future reference (pass-through writer module). HTM results are post-processed using LinearSVM classifier from scikit-learn library and visualized with matplotlib.

\paragraph{HTM Wrapper}

As mentioned above, a wrapper is created for a specific use -- the one designed to work with videos will differ from the one tailored for texts. Assembling a wrapper from predefined or newly created modules is the main task of the experiment setup.

Preparing the processing units to work is not wrapper's only responsibility -- it also controls the amount of executed iterations. The minimum (and default) cycles number equals to a single pass of the learning set, however setups specifying maximum number and/or metrics measuring if HTM still needs learning are also possible.

The wrapper module also coordinates statistics gathering and visualization on per-instance basis.

\paragraph{Adaptive Video Encoder}

During the encoding process original video frame is converted to a binary image. Depending on the configuration, the original image can be first reduced in size to trim down the amount of data. After reduction color image is converted to grayscale, which later is turned into binary one using adaptive thresholding.

Adaptive thresholding uses potentially different threshold value for each small image region. It gives better results than using single threshold value for images with varying illumination. In this encoder 'ADAPTIVE\_THRESH\_GAUSSIAN\_C' algorithm from OpenCV library is used -- a threshold value is the weighted sum of neighbourhood values where weights are a gaussian window.

\subsubsection{HTM Core}

All implemented readers, encoders, decoders and writes provide pre-defined interfaces. Such a solution allows to separate data acquisition and output storage from the actual processing. The loop consisting of data retrieval, processing and outputting is executed by the iterator object of the core module.

\paragraph{HTM}

HTM object itself consist of configurable amount of layers, spatial pooler (SP) and temporal pooler (TP) objects. Each iteration, each layer state is updated by SP and (depending on the configuration) TP, based on the data it receives. In case of the lowest layer input is obtained from encoder, for higher ones -- from the previous level. Setting layers number to zero effectively turns off HTM, causing module output to be equal to encoder one. This feature was used when comparing performance of LinearSVM only with HTM + LinearSVM ensemble.

Layers consist of columns, which are composed of connectors (containing synapses used in spatial pooling process) and cells (used in temporal pooling). Cells themselves are built from segments, with each segment containing synapses connecting it to the other cells. This hierarchical structure closely mirrors the one described in the algorithm's section.

\paragraph{Object-oriented structure}

Every object encapsulates its functionality, making introducing changes and enhancements trivial, while at the same time providing clear reference point for modifications. Object-oriented structure also enhances visibility of very important HTM's feature -- its potential for massive parallelization. One example of that can be spatial pooling process. Initial system setup used sequential version of SP, written purely in Python. After some tests, decision to replace it with concurrent implementation running on GPU (and FPGA in the future) was made. Replacement spatial pooler, taking advantage of OpenCL capabilities, was written and plugged in the system, without changes to the rest of the architecture.

